ToolNet: Connecting Large Language Models with Massive Tools via Tool Graph

While achieving remarkable progress in a broad range of tasks, large language models (LLMs) remain significantly limited in properly using massive external tools. Existing in-context learning approaches simply format tools into a list of plain text descriptions and input them to LLMs, from which, LLMs generate a sequence of tool calls to solve problems step by step. Such a paradigm ignores the intrinsic dependency between tools and offloads all reasoning loads to LLMs, making them restricted to a limited number of specifically designed tools. It thus remains challenging for LLMs to operate on a library of massive tools, casting a great limitation when confronted with real-world scenarios. This paper proposes ToolNet, a plug-and-play framework that scales up the number of tools to thousands with a moderate increase in token consumption. ToolNet organizes tools into a directed graph. Each node represents a tool, and weighted edges denote tool transition. Starting from an initial tool node, an LLM navigates in the graph by iteratively choosing the next one from its successors until the task is resolved. Extensive experiments show that ToolNet can achieve impressive results in challenging multi-hop tool learning datasets and is resilient to tool failures.

==> Fig/code_agentnet.tex <==
\fbox {
    \fontsize{7pt}{12pt}\selectfont
    
    \parbox{0.97\textwidth}
    {
        \begin{minipage}[t]{0.48\textwidth}
           \linespread{1.1} \selectfont
        \vspace{2px}
        \begin{minipage}{1.0\textwidth}
            \centering
            \textbf{ReACT}
        \end{minipage}
        
       \begin{algorithmic}[1] 
            \Function{ReACT}{$query, max\_steps, \mathcal{T}$}
                \State $context = ()$
                \State $curren\_step \leftarrow 0$
                \While {$cur < max\_steps$ or not $isFinished()$}
                    \State $action, thought \leftarrow \mathcal{M} (query, context, \mathcal{T})$
                    \State $observation \leftarrow Exec(action)$
                    \State $context \leftarrow (context, action, observation)$
                    \State $curren\_step \leftarrow curren\_step + 1$
                \EndWhile
            \EndFunction
        \end{algorithmic}
        \vspace{2px}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.48\textwidth}
           \begin{minipage}[t]{\textwidth} 
            \linespread{0.9} \selectfont
            \vspace{2px}
            \begin{minipage}{1.0\textwidth}
                \centering
                % \hspace{10px}
                \textbf{AgentNet}
            \end{minipage}
            \begin{algorithmic}[1] 
            \Function{AgentNet}{$query, max\_steps, \mathcal{T}, \pi$}
                \State $context = ()$
                \State $current\_step \leftarrow 0$
                \State $current\_action = Begin$
                \While {$cur < max\_steps$ or not $isFinished()$}
                    \State $\mathcal{T}_s \leftarrow \pi(\mathcal{T}, current\_tool)$
                    \State $action, thought \leftarrow \mathcal{M} (query, context, \mathcal{T}_s)$
                    \State $observation \leftarrow Exec(action)$
                    \State $context \leftarrow (context, action, observation)$
                    \State $current\_action \leftarrow action$
                    \State $current\_step \leftarrow current\_step + 1$
                \EndWhile
            \EndFunction
        \end{algorithmic}
        \vspace{3px}
        \end{minipage}
        \end{minipage}
    }
}

==> Fig/noisy_tools_impact.tex <==
\resizebox{0.95\textwidth}{!}{
        \begin{tabular}{cccc}
            \toprule[1.2pt]
             \multirow{2}{*}{Dataset}  &  \multirow{2}{*}{Metric} &  \multirow{2}{*}{ReACT} & ReACT \\
              & & & \small{(without noisy tools)} \\ 
            \midrule[1.2pt]
            \multirow{3}{*}{SciQA} & Win Rate & 0.45 & 0.48  \\
              &\#Tokens & 8270 & 7318 \\
              &\#Steps & 5.8 & 5.4 \\
             \midrule
            \multirow{3}{*}{TabMWP} & Win Rate & 0.26 & 0.50  \\
              &\#Tokens & 8936 & 6594 \\
              &\#Steps & 6.1 & 5.3 \\
             \midrule
             \multirow{3}{*}{MATH} & Win Rate & 0.13 & 0.20  \\
              &\#Tokens & 9216 & 8382 \\
              &\#Steps & 6.9 & 6.8 \\
            \bottomrule[1.2pt]
        \end{tabular}
}

==> Fig/result_of_large_datasets_combined.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.69\textwidth}
        
	\renewcommand{\arraystretch}{1.3}
	\centering
    \captionof{table}{Results on subsets of open-set multi-task datasets, where noisy and redundant tools inevitably exist. }
    \label{table:result_of_large_datasets}
    \resizebox{\textwidth}{!}{ 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{ccc|cccccc}
\hline
\multirow{2}{*}{Dataset}   & \multirow{2}{*}{Size} & \multirow{2}{*}{\#Tools} & \multirow{2}{*}{Metric} & \multirow{2}{*}{ReAct} & \multirow{2}{*}{Reflexion} & \multirow{2}{*}{ToT} & \multicolumn{2}{c}{ToolNet (Ours)}                                               \\ \cline{8-9} 
                           &                          &                          &                           &                        &                            &                      &  & +Reflexion \\ \hline
\multirow{2}{*}{APIBank}   & \multirow{2}{*}{212}     & \multirow{2}{*}{49}      & Win Rate                       & 0.697                  & \underline{0.767}                      & 0.629                & 0.748   & \textbf{0.834}                                                        \\
                           &                          &                          & \#Tokens                  & \underline{1720}                   & 4286                       & 2013                 & \textbf{1649}    & 3353                                                         \\ \hline
\multirow{2}{*}{ToolBench} & \multirow{2}{*}{1000}    & \multirow{2}{*}{??,3992}      & Win Rate                       & 0.607                  & 0.713                      & 0.605                & 0.687   &         ???                                                     \\
                           &                          &                          & \#Tokens                  & 8636                   & 13217                      & 10167                & 6575    &                            ???                                  \\ \hline
\end{tabular}
    }
    % \captionof{table}{Table caption}
 \label{table:result_of_large_datasets}
    \end{minipage}
    \hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Fig/dynamic_toolfail.pdf} % Replace with your figure
        \vspace{-2em}
        \caption{Resilience against sudden tool failures on ToolBench}
        \label{fig:dynamic_tool_failure}
    \end{minipage}
    % \caption{Overall results on SciQA, TabMWP, and MATH.}
\end{figure*}

==> Fig/result_of_three_datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]

	\renewcommand{\arraystretch}{1.3}
	\centering
    \caption{Overall results on scienceQA, tableMWP, MATH, and APIBank. {\color{red} Plan to move the descriptions of datasets into caption.}}
    \label{table:result_of_three_datasets}
    \resizebox{\textwidth}{!}{ 
\begin{tabular}{ccccccccc}
% \hline
\toprule[1.2pt]
Dataset & \#Cases                               & \#Tools                               & Property   & CoT                  & ReACT                      & Reflexion                      & ToolNet (Ours)                 & ToT                        \\ \hline
\multirow{3}{*}{scienceQA}      & \multirow{3}{*}{1000}                 & \multirow{3}{*}{17}                   & Acc        & 0.59                 & 0.45                       & -                              & \textbf{0.61} & 0.12                       \\
                                &                                       &                                       & \#Tokens & 1062                 & 8270                       & -                              & 5945                           & 23070                      \\
                                &                                       &                                       & \#Steps    & 1                    & 5.8                        & -                              & 4.0                            & 8.9                        \\ \hline
\multirow{3}{*}{tableMWP}       & \multirow{3}{*}{1000}                 & \multirow{3}{*}{16}                   & Acc        & 0.40                 & 0.26                       & 0.57                           & \textbf{0.67} & 0.09                       \\
                                &                                       &                                       & \#Tokens & 803                  & 8936                       & 24710                          & 4062                           & 19669                      \\
                                &                                       &                                       & \#Steps    & 1                    & 6.1                        & 11.3$^{\mathrm{*}}$            & 3.7                            & 8.7                        \\ \hline
\multirow{3}{*}{MATH}           & \multirow{3}{*}{675}                  & \multirow{3}{*}{16}                   & Acc        & 0.14                 & 0.13                       & \textbf{0.29} & 0.25                           & 0.07                       \\
                                &                                       &                                       & \#Tokens & 1410                 & 9216                       & 28886                          & 6602                           & 18090                      \\
                                &                                       &                                       & \#Steps    & 1                    & 6.9                        & 9.5                            & 5.4                            & 8.2                        \\ \cline{1-9} 
\multirow{3}{*}{APIBank}        & \multicolumn{1}{c}{\multirow{3}{*}{212}} & \multicolumn{1}{c}{\multirow{3}{*}{49}} & Acc        & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.697}  & \multicolumn{1}{c}{0.767}      & \multicolumn{1}{c}{0.748}      & \multicolumn{1}{c}{0.629}  \\
                                & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                  & \#Tokens & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1720} & \multicolumn{1}{c}{4286}     & \multicolumn{1}{c}{1649}     & \multicolumn{1}{c}{2013} \\
                                & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                  & \#Steps    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{1.8}       & \multicolumn{1}{c}{\color{red}1.8}           & \multicolumn{1}{c}{1.8}           & \multicolumn{1}{c}{1.8} \\
                                \hline
\multirow{3}{*}{ToolBench}        & \multicolumn{1}{c}{\multirow{3}{*}{1000}} & \multicolumn{1}{c}{\multirow{3}{*}{??}} & Acc        & \multicolumn{1}{c}{} & \multicolumn{1}{c}{0.607}  & \multicolumn{1}{c}{0.713}      & \multicolumn{1}{c}{0.687}      & \multicolumn{1}{c}{0.605}  \\
                                & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                  & \#Tokens & \multicolumn{1}{c}{} & \multicolumn{1}{c}{8636} & \multicolumn{1}{c}{13217}     & \multicolumn{1}{c}{6575}     & \multicolumn{1}{c}{10167} \\
                                & \multicolumn{1}{c}{}                  & \multicolumn{1}{c}{}                  & \#Steps    & \multicolumn{1}{c}{} & \multicolumn{1}{c}{5.06}       & \multicolumn{1}{c}{6.48}           & \multicolumn{1}{c}{4.76}           & \multicolumn{1}{c}{4.29} \\
    \bottomrule
\end{tabular}
    }
\end{table*}






% \begin{table*}[t]

% 	\renewcommand{\arraystretch}{1.3}
% 	\centering
%     \caption{Overall results in scienceQA, tableMWP and MATH datasets}
%     \label{table:result_of_three_datasets}
%     \resizebox{\textwidth}{!}{ 
%         \begin{tabular}{ccccccccc}
%             \toprule[1.2pt]
%              Dataset & \#Cases & \#Tools & Property & CoT & ReACT & Reflexion & ToolNet (Ours) & ToT \\
%             \midrule[1.2pt]
%             \multirow{3}{*}{scienceQA} & \multirow{3}{*}{1000} & \multirow{3}{*}{17} & Acc & 0.59 & 0.45 & - & \textbf{0.61} & 0.12\\
%              & & & #Tokens & 1062 & 8270  &  - &  5945 & 23070\\
%              & & & \#Steps & 1 & 5.8  &  - &  4.0 & 8.9\\
%              \midrule
%             \multirow{3}{*}{tableMWP} & \multirow{3}{*}{1000} & \multirow{3}{*}{16}&  Acc & 0.40 & 0.26  &  0.57 & \textbf{0.67} & 0.09\\
%              & & & #Tokens & 803 & 8936  & 24710 &  4062 & 19669 \\
%               & & & \#Steps & 1 & 6.1  &  11.3$^{\mathrm{*}}$ &  3.7 & 8.7\\
%              \midrule
%              \multirow{3}{*}{MATH} & \multirow{3}{*}{675} & \multirow{3}{*}{16} & Acc & 0.14 & 0.13 & \textbf{0.29} & 0.25 & 0.07\\
%               & & & #Tokens & 1410 & 9216 & 28886 &  6602 & 18090 \\
%               & & & \#Steps & 1 & 6.9  &  9.5 &  5.4 & 8.2\\
%             \bottomrule[1.2pt]
%             \multicolumn{4}{l}{$^{\mathrm{*}}$ Total steps in all trials of Reflexion.}
%         \end{tabular}
%     }
% \end{table*}


% \begin{tabular}{cccccccc}
%     \toprule
%      Dataset & Property & CoT & ReACT & ReACT (Good Tools) & Reflexion & AgentNet & ToT \\
%     \midrule
%     \multirow{2}{*}{sciQA} & Acc & 0.59 & 0.45 & 0.49 & - & \textbf{0.61} & 0.12\\
%     & #Tokens & \textbf{1062} & 8270  & 7318 & - &  5945 & 23070\\
%     \bottomrule
%     \multirow{2}{*}{tableMWP} & Acc & 0.40 & 0.26 & 0.50 &  0.57 & \textbf{0.67} & 0.09\\
%     & #Tokens & \ \textbf{803} & 8936 & 6594 & 24710 &  4062 & 19669 \\
%     \bottomrule
%     \multirow{2}{*}{MATH} & Acc & 0.14 & 0.13 & 0.20 & \textbf{0.29} & 0.25 & 0.07\\
%     & #Tokens & 1410 & 9216 & 8382 & 28886 &  6602 & 18090 \\
%     \bottomrule
% \end{tabular}

==> Fig/result_of_toy_datasets_combined.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.65\textwidth}
        
	\renewcommand{\arraystretch}{1.3}
	\centering
    \captionof{table}{Results on subsets of close-set task-specific datasets. Noisy and task-irrelevant tools, as described in Table.\ref{table:three_datasets_tools}, are introduced to analyze the robustness of prompting paradigms. Reflexion is not evaluated on SciQA, a multiple-choice QA dataset, as it would not provide a fair comparison.}
    \label{table:result_of_toy_datasets}
    \resizebox{0.5\textwidth}{!}{ 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lC{0.5cm}C{0.5cm}|cccccc}
\toprule
Dataset & Size               & \#Tools             & Metric  & ReAct & \begin{tabular}[c]{@{}c@{}}ReAct\\ ({clean})\end{tabular} & Reflexion                      & ToT   & \begin{tabular}[c]{@{}c@{}}ToolNet\\ (\textbf{Ours})\end{tabular}                 \\ \hline
\multirow{3}{*}{SciQA} & \multirow{3}{*}{1000} & \multirow{3}{*}{16} & EM      & 0.45 & 0.48 & -                              & 0.12  & \textbf{0.61} \\
                           &                       &                     & \#Tokens  & 8270  & 7318 & -                              & 23070 & \underline{5945}                           \\
                           &                       &                     & \#Steps  & 5.8  & 5.4 & -                              & 8.9   & 4.0                            \\ \hline
\multirow{3}{*}{TabMWP}  & \multirow{3}{*}{1000} & \multirow{3}{*}{16} & EM  & 0.26  & 0.50 & \underline{0.57}                           & 0.09  & \textbf{0.67} \\
                           &                       &                     & \#Tokens  & 8936 & 6594 & 24710                          & 19669 & \underline{4062}                           \\
                           &                       &                     & \#Steps  & 6.1  & 5.3 & 11.3$^{\mathrm{*}}$            & 8.7   & 3.7                            \\ \hline
\multirow{3}{*}{MATH}      & \multirow{3}{*}{675}  & \multirow{3}{*}{16} & EM     & 0.13 & 0.20  & \textbf{0.29} & 0.07  & \underline{0.25}                           \\
                           &                       &                     & \#Tokens  & 9216 & 8382 & 28886                          & 18090 & \underline{6602}                           \\
                           &                       &                     & \#Steps    & 6.9 & 6.8  & 9.5                            & 8.2   & 5.4           \\                 \bottomrule
\end{tabular}
    }
    % \captionof{table}{Table caption}
 \label{tab:table1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.34\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Fig/three_toy_dataset_fig.pdf} % Replace with your figure
        \vspace{-2em}
        \caption{Scores of
tools in SciQA, TabMWP, and MATH in dynamic graph construction. Tools effective for task-specific datasets have increasing scores.}
        \label{fig:figure1}
        % \centering
        % \begin{minipage}[t]{0.2\textwidth}
        %     \begin{minipage}[t]{0.2\textwidth}
        %     \captionsetup[subfloat]{captionskip=0pt, labelformat=empty}
        %     \subfloat[\hspace{1em} (a) SciQA]
        %     {
        %         \input{Fig/experiment_figures/sciQA_tools_scores_revised}
        %     }
        %     \end{minipage}
        %     \begin{minipage}[t]{0.2\textwidth}
        %     \captionsetup[subfloat]{captionskip=0pt, labelformat=empty}
        %     \subfloat[\hspace{1em} (b) TabMWP]
        %     {
        %         \input{Fig/experiment_figures/tableMWP_tools_scores_revised}
        %     }
        %     \end{minipage}
        %     \begin{minipage}[t]{0.2\textwidth}
        %     \captionsetup[subfloat]{captionskip=0pt, labelformat=empty}
        %     \subfloat[\hspace{-7em} (c) MATH]
        %     {
        %         \input{Fig/experiment_figures/math_tools_scores_revised}
        %     }
        %     \end{minipage}    
        % \end{minipage}
    \end{minipage}
    % \caption{Overall results on SciQA, TabMWP, and MATH.}
\end{figure*}
